Geometric Tiles and Powers and Limitations of Geometric Hindrance in Self-Assembly

Tile-based self-assembly systems are capable of universal computation and algorithmically-directed growth. Systems capable of such behavior typically make use of "glue cooperation" in which the glues on at least $2$ sides of a tile must match and bind to those exposed on the perimeter of an assembly for that tile to attach. However, several models have been developed which utilize "weak cooperation", where only a single glue needs to bind but other preventative forces (such as geometric, or steric, hindrance) provide additional selection for which tiles may attach, and where this allows for algorithmic behavior. In this paper we first work in a model where tiles are allowed to have geometric bumps and dents on their edges. We show how such tiles can simulate systems of square tiles with complex glue functions (using asymptotically optimal sizes of bumps and dents), and also how they can simulate weakly cooperative systems in a model which allows for duples (i.e. tiles either twice as long or twice as tall as square tiles). We then show that with only weak cooperation via geometric hindrance, no system in any model can simulate even a class of tightly constrained, deterministic cooperative systems, further defining the boundary of what is possible using this tool.

==> duples-cannot-sim-gtam.tex <==
\section{Duples Cannot Simulate GTAM Systems}\label{sec:imposs-duples}

We now show that there exist GTAM systems which cannot be simulated by any DaTAM system. At a high-level, the reason for this is that the placement of a GTAM tile can have two properties: (1) it exposes geometry on its output sides which prevent the placement of (at least some types of) tiles adjacent to those output sides, and (2) this geometric hindrance is simultaneously enforced on opposite sides of the tile. Because of this, any simulating system would need to grow macrotiles which can prevent the growth of some neighbors, but since it's impossible to do so without placing tiles in multiple distributed locations, and multiple tiles cannot be placed simultaneously, it must be possible for assemblies to exist in the simulator in which either: (1) a location which maps to empty space is preventing other locations from growing into some types of macrotiles, or (2) a location which maps to a tile which should be preventing the growth of neighbors into some types, doesn't always do so. Either situation is a failure to correctly simulate. An overview of the GTAM system which cannot be simulated can be seen in Figure~\ref{fig:duple-imposs-overview}, and the particular locations which cause simulation by duples to fail can be seen in Figure~\ref{fig:arm-cup}, and are labeled at $a$, $b$, and $x$. The full proof can be found in the Appendix.

\begin{theorem}\label{thm:imposs-geo}
There exists a GTAM system $\calG$ which cannot be simulated by any DaTAM system.
\end{theorem}

\begin{figure}
    \centering
    \includegraphics[width=4.5in]{figures/GTAM-all-growth.png}
    \caption{Overview of a GTAM system $\calG$ which cannot be simulated by any DaTAM system. The seed is the black tile in the left column, and the white locations surrounded by dashed lines haven't yet received tiles.}
    \label{fig:duple-imposs-overview}
\end{figure}

% \begin{figure}
%     \begin{center}
%         \begin{tikzpicture}[x=0.5cm, y=0.5cm]
%             \def\x{0}
%             \def\y{0}
%             \draw[dashed] (\x+1,\y+3)--(\x+4,\y+3) (\x+1,\y+4)--(\x+4,\y+4) (\x+2,\y+3)--(\x+2,\y+4) (\x+3,\y+3)--(\x+3,\y+4);
%             \fill[fill=gray!70!white] (\x+2,\y) -- (\x+2,\y+1) -- (\x,\y+1) -- (\x,\y+4) -- (\x+1,\y+4) -- (\x+1,\y+2) -- (\x+4,\y+2) -- (\x+4,\y+4) -- (\x+5,\y+4) -- (\x+5,\y+1) -- (\x+3,\y+1) -- (\x+3,\y) -- (\x+2,\y);
%             \draw (\x+2,\y) -- (\x+2,\y+1) -- (\x,\y+1) -- (\x,\y+4) -- (\x+1,\y+4) -- (\x+1,\y+2) -- (\x+4,\y+2) -- (\x+4,\y+4) -- (\x+5,\y+4) -- (\x+5,\y+1) -- (\x+3,\y+1) -- (\x+3,\y);
%             \fill[fill=gray!70!white] (\x+2,\y+6)--(\x+2,\y+4)--(\x+3,\y+4)--(\x+3,\y+6)--(\x+2,\y+6);
%             \draw (\x+2,\y+6)--(\x+2,\y+4)--(\x+3,\y+4)--(\x+3,\y+6);
%             \node at (\x+1.5,\y+3.5) {a};
%             \node at (\x+2.5,\y+3.5) {x};
%             \node at (\x+3.5,\y+3.5) {b};
%         \end{tikzpicture}
%     \end{center}
%     \caption{An arm and cup in $\calG$ without any of the five center tiles, but with their locations outlined and labeled.}
%     \label{fig:arm-cup}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=1.9in]{figures/GTAM-bottom-gadgets.png}
%     \caption{The bottom gadgets of the GTAM system.}
%     \label{fig:gtam-bottom-gadets}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=4.5in]{figures/GTAM-top-gadgets.png}
%     \caption{The top gadgets of the GTAM system.}
%     \label{fig:gtam-bottom-gadets}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=4.5in]{figures/GTAM-bottom-growth.png}
%     \caption{The initial growth of just a series of bottom gadgets of the GTAM system.}
%     \label{fig:gtam-bottom-growth}
% \end{figure}



==> proofs2.tex <==
\subsection{Proof of Theorem~\ref{thm:imposs-geo}}

Here's the high-level organization of the proof, which we'll obviously need to formalize more. The general procedure will be to run an assembly of $\calG$ to specified points by selecting valid assembly sequences which arrive at target shapes. We'll then have the simulation by $\calD$ proceed to the point of matching that assembly (which must be possible if $\calD$ simulates $\calG$), and we'll inspect and record subsequences of the assembly process. This will eventually allow us to prove that $\calD$ has to perform growth which violates the definition of simulation.
\begin{enumerate}
    \item Initialize $\calG$ to begin from its single seed tile, and the simulation $\calD$ to begin from the single macrotile representing that seed. Let $m$ be the scale factor by which $\calD$ simulates $\calG$.
    
    \item Define the \emph{pumping distance} in $\calD$ to be  $p = ((g+1)^{6m}\cdot(6m)!+1)\cdot$, where $g$ is the number of glues in $D$\todo{Give an explanation for this choice}
    
    \item Run $\calG$ so that it grows only upward from the seed and then grows eastward, fully completing each downward growing arm before continuing east. Have it grow to the point that it has completed growth of $p$ arms. See Figure~\ref{fig:GTAM-top-growth-pattern} for an example of the pattern of growth for one section containing an arm.
    
    \item Now run $\calD$ so that it simulates the same assembly sequence up until the point that it places the very first tile which causes the assembly representation function $R^*$ to resolve the final tile which was placed in $\calG$. Record the full assembly sequence, which we'll refer to as $S_{\texttt{top}}$. Furthermore, during the assembly process, record every window movie across the vertical cuts to the immediate right side of each yellow tile of the upper arm (see Figure~\ref{fig:GTAM-top-windows} for an example).
    
    \item By our choice of the value $p$, it must be the case that at least two of the vertical cuts, which we'll refer to as \emph{windows} (see \cite{IUNeedsCoop}), have the same window movie, which means that they have the same glues placed along them, in the same order. Call the leftmost copy of the window $w_0$, and the rightmost $w_1$.
    
    \item We now rewind $\calD$ until it has placed the first tile across $w_1$, and we let $S_{\texttt{top-pump}}$ be the portion of assembly sequence $S$ which contains all tile placements from the first tile placed across $w_0$ to the first tile placed across $w_1$. Since $w_0$ and $w_1$ had identical window movies in $S$, then either (1) on the left side of $w_1$ is the same set of tiles which were to the left of $w_0$ when the first tile was placed to its right, or (2) some path(s) of tiles crossed both windows after the first tile crossed $w_1$, but that means that there's a valid assembly sequence beginning from tiles attaching to those on the left of $w_0$ up until placing the first tile across $w_1$, and we let $S_{\texttt{top-pump}}$ be just that. Since $S_{\texttt{top-pump}}$ was a valid assembly (sub)sequence which grew from $w_0$ to $w_1$ in this state, it is possible to repeat $S_{\texttt{top-pump}}$ an arbitrary number of additional times, which we will refer to as \emph{pumping} the top half of the assembly. We'll refer to the first arm to grow downward after each pump to be $\texttt{arm}_0$, and we'll note that each copy of $\texttt{arm}_0$ contains exactly the same tiles placed in exactly the same order. (An arm consists of a downward growing column of two grey tiles and one green tile, as seen in Figure~\ref{fig:GTAM-top-windows}.) In fact, if $n$ is the number of yellow tiles between $w_0$ and $w_1$, then there are $n$ arms in each pumped segment, and for each $0 \le i < n$, the $i$th arm of each pumped segment is identical.
    
    \item Note that whenever we rewind, grow, or pump $\calD$, we do the same to $\calG$ to keep them in sync.
    
    \item TODO: more detail here.  Now we'll grow the bottom out until it similarly pumps. However, we'll also have to watch for any paths which grow through the seed macrotile or its surrounding fuzz.  We'll essentially start over with our top pumping whenever that happens, noting that it can only happen at most $3m$ times.
    
    \item TODO: more detail here. Eventually, we will have independently pumping arms and cups, meaning that both can be pumped and grown completely independently of each other. We will then grow them out to the same distance, and then grow an arm and cup which haven't placed any of the center tiles, and we'll record the location of the point of competition (POC).
    
    \item TODO: more detail here. We'll argue that the POC must be in the same location every time that same copy of the arm grows. Now we'll show that it must be in one of the geometry regions to the left of right of the macrotile representing $x$ (the green tile).
    
    \item TODO: more detail here. Maybe we'll find the POC for each of the $n$ arms in the pumpable segment.
    
    \item TODO: more detail here. If the POCs of different arms are on different sides, left or right, we'll choose the left as our ``target'' side.  If they are all on the same side, we'll use that as our side. Without loss of generality, assume that the left is our target side.
    
    \item TODO: more detail here. We'll now pump the bottom out (beyond the distance that the top has grown, until we find a new pumpable segment), but this time we will only grow the right side of each cup, including the macrotiles in locations $c$ and $d$. Once we've found a pumpable segment, we'll record the growth of the $c$ and $d$ macrotiles of each cup in that segment.
    
    \item TODO: more detail here. We will then grow the top and bottom out to the same distance by (partially if necessary at the end) pumping them. Once they are aligned, we will grow a complete arm, with its $x$ macrotile. We'll then grow the cup, and as it grows the right arm and attempts to grow $d$ then $c$, we'll find that either (1) it is able to do so, breaking the simulation since $x$ is incompatible with $c$, or (2) it will have to grow down through the cup and up into empty space where the left side should have been (since that is the only path to the POC - which is the only thing that can stop its growth - because when we recorded the growth of $c$ and $d$ previously, we noted that no growth went into the location of $x$'s body since that would have broken fuzz, and thus the simulation), again breaking simulation. 
    
\end{enumerate}

\begin{proof}
We will define GTAM system $\calG = (G,\sigma_{\calG},1)$, and then prove Theorem~\ref{thm:imposs-geo} by contradiction. To do so, we will assume that $\calD = (D,\sigma_{\calD}, 1)$ is a DaTAM system which correctly simulates $\calG$ and then show why that assumption must fail.

Let $\calG$ be the temperature-1 GTAM system which begins growth from a single seed tile (shown in black in the left column of Figure~\ref{fig:duple-imposs-overview}). It produces an infinite assembly in which top and bottom ``arms'' each extend infinitely far.  From the seed, the top arm grows upward a distance of four tiles, then grows infinitely far to the right. Also, starting from the eighth tile, every tenth tile position in the top arm grows a short arm downward. From the seed, the bottom arm grows down a distance of four tiles, and then grows infinitely far to the right. Also, starting from the eight tile, every tenth tile position in the bottom arm grows a small ``cup'' assembly upward. Figure~\ref{fig:duple-imposs-overview} shows an overview of a portion of a terminal assembly (with some missing tiles), and a zoomed in view of an arm and cup can be seen in Figure~\ref{fig:arm-cup}. Note that in both figures, none of the possible tiles that could fit into the five locations at the top of a cup have attached. They will be explained in more detail later. Now we suppose that there exists some temperature-1 DaTAM system $\calD = (D,\sigma_{\calD}, 1)$ which simulates $\calG$ using a scale factor $m$ for the $m \times m$ tile bodies and $n \times m$ rectangles for the geometry regions.

\begin{figure}
    \centering
    \includegraphics[width=4.5in]{figures/GTAM-top-growth-pattern.png}
    \caption{Series of images showing, from left to right and top to bottom, the ordering of growth of one portion of $\calG$ containing an arm}
    \label{fig:GTAM-top-growth-pattern}
\end{figure}

Throughout this proof we will consider a variety of assembly sequences in $\calG$ and investigate corresponding assembly sequences in $\calD$. First consider the assembly sequence $\Vec{\alpha_\texttt{top}}$ which begins at the seed assembly $\sigma_\calG$ and begins growth upward and to the east, growing each vertical arm fully before continuing. This growth continues until a sufficiently large number of arms, say $p$, have grown. Figure \ref{fig:GTAM-top-growth-pattern} illustrates this growth pattern. Consider then any corresponding assembly sequence, say $\Vec{\beta_\texttt{top}}$, in $\calD$, wherein the macrotiles resolve in the exact same order as the tiles grown in $\Vec{\alpha_\texttt{top}}$. Such an assembly sequence must exist since $\calD$ simulates $\calG$.

We define a \emph{window} to be any cut of the square lattice. Because every binding graph of an assembly is a subgraph of the square lattice, a window may intersect the edges of a binding graph. In terms of tile assembly, this represents a path between tiles which divides an assembly into two pieces. During any individual assembly, a window might cross a number of glues between adjacent tiles. If we consider the glues along a window during the course of an assembly sequence, we get a \emph{window movie}. Consider the tiles illustrated in yellow in figure \ref{fig:GTAM-top-growth-pattern} and notice that there are only a finite number of ways in which tiles can be placed along the east face of a macrotile in $\calD$ representing such a yellow tile in $\calG$, even taking into account the order in which the tiles are placed. In other words there are only a finite number of window movies which can occur along the vertical cuts which divide the assembly right after the yellow macrotiles. Such cuts are illustrated in figure \ref{fig:GTAM-top-windows}. Note that to be guaranteed to cut the assembly into two portions the windows must be of at least height $3m + 4n$ to cross the macrotile representing a tile, plus the macrotiles allowed for fuzz above and below, plus the corresponding regions to represent the geometry regions. Additionally, the windows may be jagged to accommodate duples. Nonetheless, there remain a finite number of such possible cuts given the finite number of tile types and glues in $D$.

\begin{figure}
    \centering
    \includegraphics[width=4.5in]{figures/GTAM-top-windows.png}
    \caption{Example depiction of two cuts (black vertical lines) along two identical windows}
    \label{fig:GTAM-top-windows}
\end{figure}

Since there are only a finite number of such window movies, if we choose $p$ to be large enough so that sufficiently many arms, and thus yellow tiles, have grown, then it must be the case that two of these window movies in $\Vec{\beta_\texttt{top}}$ are identical. This means that the tiles, and the relative order in which they grew, along the east face of two distinct yellow macrotiles must be identical. We will call the leftmost of a pair of identical windows $w_0$, and the rightmost $w_1$.

We now rewind $\calD$ until it has placed the first tile across $w_1$, and we let  $\Vec{\beta_\texttt{top-pump}}$ be the portion of assembly sequence  $\Vec{\beta_\texttt{top}}$ which contains all tile placements from the first tile placed across $w_0$ to the first tile placed across $w_1$. Since $w_0$ and $w_1$ had identical window movies in  $\Vec{\beta_\texttt{top}}$, then either (1) on the left side of $w_1$ is the same set of tiles which were to the left of $w_0$ when the first tile was placed to its right, or (2) some path(s) of tiles crossed both windows after the first tile crossed $w_1$, but that means that there's a valid assembly sequence beginning from tiles attaching to those on the left of $w_0$ up until placing the first tile across $w_1$, and we let  $\Vec{\beta_\texttt{top-pump}}$ be just that. Since  $\Vec{\beta_\texttt{top-pump}}$ was a valid assembly (sub)sequence which grew from $w_0$ to $w_1$ in this state, it is possible to repeat  $\Vec{\beta_\texttt{top-pump}}$ an arbitrary number of additional times, which we will refer to as \emph{pumping} the top half of the assembly. We'll refer to the first arm to grow downward after each pump to be $\texttt{arm}_0$, and we'll note that each copy of $\texttt{arm}_0$ contains exactly the same tiles placed in exactly the same order. (An arm consists of a downward growing column of two grey tiles and one green tile, as seen in Figure~\ref{fig:GTAM-top-windows}.) In fact, if $x$ is the number of yellow tiles between $w_0$ and $w_1$, then there are $x$ arms in each pumped segment, and for each $0 \le i < x$, the $i$th arm of each pumped segment is identical.

%Because these window movies are identical, it must be possible, in $\calD$, for the assembly to the east of the first such macro tile to grow from the presented tiles of the second macrotile. \todo{maybe cite WML and say that the reasoning is similar}. This means that for sufficiently long $\Vec{\alpha_\texttt{top}}$ there are corresponding assembly sequences in $\calD$ wherein the representations of the vertical arms are periodic after some finite distance. We call this $\emph{pumping}$ the top half of the assembly.

Now consider any assembly sequence $\Vec{\alpha_\texttt{bottom}}$ in $\calG$ where we start with the seed assembly $\sigma_\calG$ and grow downward and east, making sure to finish each cup before continuing east. Notice that when constructing a cup there is a choice in the order in which the halves of the cups are constructed. Regardless, of this choice, the same pumping argument can be made for a corresponding assembly sequence in $\calD$. Next, we can consider any assembly sequence $\Vec{\alpha_\texttt{both}}$ in $\calG$ which first grows the top half of the assembly sufficiently far, making sure to complete all arms before continuing east. Note that we can guarantee that our top half grows far enough so that, when simulated in $\calD$, the top pumps sufficiently many times noting that the period of pumped sections can be limited by some value, say $n$, which depends on the fixed scale factor of the simulation. Then, after the growth of the top, we grow the bottom half so that we grow only half of each cup before continuing eastward. For the first $n$ cups we grow only the left half and the tiles in $a$ and $b$ and for the next $n$ cups we grow only the right half and the tiles in $c$ and $d$. We then alternate this pattern. 

% Growth of the GTAM system which must be simulated:
% \begin{enumerate}
%     \item Define a pumping length $c$ for the simulating system
%     \item First the bottom grows an aperiodic series of bottom gadgets of at least length $c$ gadgets
%     \item Then the column grows upward from the seed at least length $c$
%     \item The red tile gets nondeterministically placed to cap the upward growth of the left column
%     \item The top bar grows in a pattern of growing to an orange location, growing down distance $c$, then continuing growth to the right to the next orange location, growing down a distance of $c$, etc., until $c$ orange locations have been passed
%     \item We now pump the top out $cm$ times (where $m$ is some big number to be defined)
%     \item Looking at each of the $m$ new copies of the arm which grew down, we note that they are identical and can all be pumped, and pump each (using identical assembly sequences) until the first tile which causes the tile above the point of collision to be represented
%     \item We can guarantee that of the $m$ arms, there is at least one above each of the $4$ types of bottom gadgets
%     \item Now for the analysis of paths...
% \end{enumerate}

\begin{figure}
    \begin{center}
        \begin{tikzpicture}[x=0.5cm, y=0.5cm]
            \def\x{0}
            \def\y{0}
            \draw[dashed] (\x+1,\y+3)--(\x+6,\y+3) (\x+1,\y+4)--(\x+6,\y+4) (\x+2,\y+3)--(\x+2,\y+4) (\x+3,\y+3)--(\x+3,\y+4) (\x+4,\y+3)--(\x+4,\y+4) (\x+5,\y+3)--(\x+5,\y+4);
            \fill[fill=gray!70!white] (\x+3,\y) -- (\x+3,\y+1) -- (\x,\y+1) -- (\x,\y+4) -- (\x+1,\y+4) -- (\x+1,\y+2) -- (\x+6,\y+2) -- (\x+6,\y+4) -- (\x+7,\y+4) -- (\x+7,\y+1) -- (\x+4,\y+1) -- (\x+4,\y) -- (\x+3,\y);
            \draw (\x+3,\y) -- (\x+3,\y+1) -- (\x,\y+1) -- (\x,\y+4) -- (\x+1,\y+4) -- (\x+1,\y+2) -- (\x+6,\y+2) -- (\x+6,\y+4) -- (\x+7,\y+4) -- (\x+7,\y+1) -- (\x+4,\y+1) -- (\x+4,\y);
            \fill[fill=gray!70!white] (\x+3,\y+6)--(\x+3,\y+4)--(\x+4,\y+4)--(\x+4,\y+6)--(\x+3,\y+6);
            \draw (\x+3,\y+6)--(\x+3,\y+4)--(\x+4,\y+4)--(\x+4,\y+6);
            \node at (\x+1.5,\y+3.5) {a};
            \node at (\x+2.5,\y+3.5) {b};
            \node at (\x+3.5,\y+3.5) {x};
            \node at (\x+4.5,\y+3.5) {c};
            \node at (\x+5.5,\y+3.5) {d};
            
            \node at (\x+5,\y+5.5) {Arm};
            \node at (\x+8,\y+2.5) {Cup};
        \end{tikzpicture}
    \end{center}
    \caption{An arm and cup in $\calG$ without any of the five center tiles, but with their locations outlined and labeled.}
    \label{fig:arm-cup}
\end{figure}

% We now discuss the possible growth of tiles into a cup of $\calG$ and refer to Figure~\ref{fig:arm-cup} for clarification.
% In $\calG$, the location $a$ can only become one tile type, $A$, which is grown from the glue presented to its West. Likewise, location $d$ can only become one tile type, $D$, which is grown from the glue presented to its East. Locations $b$ and $c$ can each become one of two tiles non-determinisically, namely $B_0$ and $B_1$ for $b$ and $C_0$ and $C_1$ for $c$. Both $B_0$ and $B_1$ grow from the East glue presented by tile $A$ once it grows and likewise for tiles $C_0$ and $C_1$ from $D$. Location $x$ can become only one tile, $X$, which grows from the glue presented to its North. Furthermore, let $X$ be geometrically incompatible on its West and East with $B_0$ and $C_0$ respectively. Thus if one of them attaches, $X$ cannot and vice-versa. Since $X$ is not incompatible with $B_1$ and $C_1$, assemblies which do grow tile $X$ will eventually grow tiles $B_1$ and $C_1$ in locations $b$ and $c$ respectively.

We now discuss the possible growth of tiles into a cup of $\calG$ and refer to Figure~\ref{fig:arm-cup} for clarification.
In $\calG$, the location $a$ can only become one tile type, $A$, which is grown from the glue presented to its West. Likewise, location $d$ can only become one tile type, $D$, which is grown from the glue presented to its East. Location $b$ can only become one tile type, $B$ which is grown from a glue on the East of tile type $A$, and likewise for location $c$ with a glue from the West of tile type $D$. Location $x$ can become only one tile, $X$, which grows from the glue presented to its North. Furthermore, let $X$ be geometrically incompatible on its West and East with $B$ and $C$, respectively. Thus if one of them attaches, $X$ cannot and vice-versa.

% Let $\alpha$ be an assembly in $\calG$, a subassembly of which is depicted in Figure \ref{fig:arm-cup}, and $\alpha'$ be the assembly $\alpha$ with the addition of a tile of type $X$ in location $x$. Also, let $\beta$ be some assembly in $\calD$ that represents $\alpha$ and $\beta'$ be some assembly in $\calD$ that represents $\alpha'$, where there exists an assembly sequence such that $\beta \rightarrow^\mathcal{D} \beta'$ (such a pair of assemblies must exist since $\calD$ simulates $\calG$). Also let $a'$ be the macrotile location in assemblies of $\calD$ corresponding to the tile location $a$ in $\calG$ and likewise for each of the other tile locations, using a prime symbol to signify a macrotile version of a tile location.

\begin{lemma}
    Let $\alpha$ is an assembly in $\calG$ wherein an arm has grown but none of $a$, $b$, $c$, $d$, or $x$ have, and let $\alpha'$ be the assembly in $\calG$ wherein $x$ has grown and $\alpha\to^\calG\alpha'$. Also let $\beta$ and $\beta'$ be assemblies in $\calD$ such that $R^*(\beta)=\alpha$, $R^*(\beta')=\alpha'$, and $\beta\to^\calD\beta'$. If $S=\{\beta_1,\ldots,\beta_n\}$ is any assembly sequence where $\beta_1=\beta$ and $\beta_n=\beta'$, then there must be some assembly, say $\beta_i$, in $S$ which satisfies the following properties:
    \begin{enumerate}
        \item Any assembly producible from $\beta_i$ cannot resolve $b'$,
        \item Any assembly producible from $\beta_i$ cannot resolve $c'$, and
        \item Any assembly producible from $\beta_i$ must resolve $x'$.
    \end{enumerate}
    Furthermore, it must be the case that the preceding assembly, say $\beta_{i-1}$ must satisfy:
    \begin{enumerate}
        \item There are assemblies producible from $\beta_{i-1}$ which resolve $b'$,
        \item There are assemblies producible from $\beta_{i-1}$ which resolve $c'$, and
        \item There are terminal assemblies producible from $\beta_{i-1}$ wherein $x'$ does not resolve.
    \end{enumerate}
\end{lemma}

\begin{proof}
Let $S=\{\beta_1,\ldots,\beta_n\}$ be any such assembly sequence from $\beta$ to $\beta'$. We'll note the existence of three special assemblies in $S$. First, consider the first assembly in $S$, say $\beta_i$, such that for every assembly $\gamma \in \prodasm{\calD}$ wherein $R(b')$ is defined (a.k.a. resolves, or maps to a tile type rather than empty space), it cannot be that $\beta_i\to^\calD\gamma$. In other words, $\beta_i$ is the first assembly in $S$ such that no producible assemblies in any assembly sequence continuing from $\beta_i$ (not necessarily just $S$), will resolve $b'$. Notice that such an assembly must exist in $S$ because $\beta_1$ does not satisfy the property while $\beta_n$ does. Furthermore any assembly which is producible beginning from $\beta_i$ will satisfy this property. Second, consider the first assembly in $S$, say $\beta_j$, such that for every assembly $\gamma \in \prodasm{\calD}$ wherein $R(c')$ is defined, it cannot be that $\beta_i\to^\calD\gamma$. This is defined identical to $\beta_i$ but with macrotile location $c'$ instead of $b'$. Third and finally, consider the first assembly in $S$, say $\beta_k$, such that for every terminal assembly $\gamma \in \prodasm{\calD}$ wherein $R(x')$ is undefined, it cannot be that $\beta_j\to^\calD\gamma$; that is, $\beta_k$ is the first assembly such that no producible terminal assemblies of any valid assembly sequence continuing from $\beta_k$ can leave $x'$ unresolved. Again, this property is not satisfied by $\beta_1$, but is satisfied by $\beta_n$, and any assembly with this property yields assemblies with this property, so such a $\beta_k$ must exist.

Now we will show that in $S$, $\beta_i$ must be the same assembly as $\beta_j$ and $\beta_k$. We start by showing that $\beta_i=\beta_j$. For contradiction, suppose that $i<j$, that is $\beta_i$ comes before $\beta_j$ in $S$. If this were the case, then once we reached $\beta_i$ in $S$, it would be possible to produce an assembly wherein $c'$ resolves since we haven't yet reached $\beta_j$. Formally, there would exist an assembly $\gamma\in\prodasm{\calD}$ wherein $R(c')=C$ such that $\beta_i\to^\calD\gamma$. Notice though that after $c'$ resolves, it would be impossible for $x'$ to resolve and thus $b'$ must resolve at some point in the future. This, however, contradicts the definition of $\beta_i$ and so $\beta_i\ge\beta_j$. Since this logic applies in the other direction too, it must be that $\beta_i=\beta_j$.

Now, for contradiction, suppose that $i<k$, that is $\beta_i$ comes before $\beta_k$ in $S$. If this were the case, then once we reached $\beta_i$ in $S$, it would still be possible to produce terminal assemblies wherein $x'$ does not resolve since we haven't yet reached $\beta_k$. Formally, there would exist an assembly $\gamma\in\termasm{\calD}$ wherein $R(x')$ is undefined and $\beta_i\to^\calD\gamma$. Notice, though, that if $x'$ never resolves in $\gamma$, $b'$ and $c'$ must, since otherwise $\gamma$ would not represent a terminal assembly but would itself be terminal. This is a contradiction, however, since $\beta_i$ was defined so that from it there are no producible assemblies where $b'$ or $c'$ resolved. This demonstrates that $k\le i$. Additionally, for contradiction, suppose that $k<i$. If this were the case, then once we reached $\beta_k$ in $S$, it would still be possible to produce assemblies wherein $b'$ or $c'$ resolve since we haven't reached $\beta_i$ yet. This means that there exists an assembly $\gamma\in\prodasm{\calD}$ wherein either (or both) $R(b')=B$ or $R(c')=C$, without loss of generality assume $R(b')=B$. Since $b'$ has resolved, it must be the case that any producible assembly leaves $x'$ unresolved since they are incompatible. This contradicts the definition of $\beta_k$, however, and so it must be that $\beta_i=\beta_k$. This demonstrates that the assembly $\beta_i=\beta_j=\beta_k$ satisfies the desired properties. Furthermore, notice that this lemma does not require that a cup has fully grown yet. \qed
\end{proof}

\todo{DH: with this lemma in place, we need to discuss the pumping and show that $C$, if it tries to check the single tile between $X$ and $B$, must grow out of fuzz. The following paragraph is invalid, but might be a template for the conclusion}

This means that the assembly $\beta_i$ represents a point in the assembly sequence $S$ after which all assemblies must resolve $x'$ and no assemblies can resolve $a'$ or $b'$. Moreover, it must be the case that in the assembly immediately preceding $\beta_i$, say $\beta_{i-1}$, there must be producible assemblies wherein $x'$ never resolves and producible assemblies wherein $a'$ or $b'$ can resolve. Notice though, that between $\beta_{i-1}$ and $\beta_i$ only a single tile, say $t$, is placed. This is problematic as this tile must influence the growth of both $a'$ and $d'$. To see this, let $\gamma_A$ be an assembly wherein $A$ is represented and $\beta_{i-1}\to^\calD\gamma_A$; such an assembly must exist because, by the definition of $\beta_{i-1}$, there exist producible assemblies where $a'$ resolves. Likewise let $\gamma_B$ be an assembly wherein $B$ has resolved and $\beta_{i-1}\to^\calD\gamma_B$. Because either of these assemblies are exclusive to any assembly wherein $X$ has grown, since $X$ is geometrically incompatible with $A$ and $B$, the placement of tile $t$ must prevent both of these assemblies from growing. We now show that no such single location exists.
There is, however, no location where $t$ can be placed so as to prevent the growth of both assembly sequences. (Need to invoke identical representations and WML) \qed

\end{proof}

Theorem~\ref{thm:imposs-geo} shows that it is impossible for DaTAM systems to simulate all GTAM systems. As previously mentioned, this is due to the ability of individual GTAM tiles to instantaneously block the growth of multiple adjacent tiles, but simulating systems of DaTAM tiles cannot perform the tile placements necessary for such distributed blocking simultaneously. However, the proof we have provided makes use of restrictions enforced by the definitions of simulation which we use, such as the restricted distance for the growth of fuzz.  While these are standard definitions used for both positive and negative results, a more general proof would be preferred.  We conjecture that, especially for temperature-1 simulators, it is possible to show that invalid assemblies can always be created by the simulators, namely assemblies form whose macrotiles map into mutually incompatible tile placements. However, such a proof seems to require significantly more case analysis, and is beyond the scope of this version of the paper.



 
% \begin{lemma}
%     Let $\alpha$ be the assembly representing the arm and cup assembly in $\calG$ depicted in figure \ref{fig:arm-cup} and $\alpha'$ be the assembly $\alpha$ with the tile $X$ in position $x'$.
%     Also let $\beta$ be an assembly in $\calD$ that represents $\alpha$ and $\beta'$ be an assembly in $\calD$ that represents $\alpha'$. In any assembly sequence $S$ from $\beta$ to $\beta'$, there must be a first assembly $\beta_i$ in $S$ such that:
%     \begin{itemize}
%         \item No assembly producible from $\beta_i$
%     \end{itemize}
% \end{lemma}
